Breaking Universality in the Lower Order Terms in the 1-level and 2-level Density of Holomorphic Cusp Newforms

The Katz--Sarnak density conjecture predicts that the normalized low-lying zeros of a family of $L$-functions ordered by analytic conductor $R$ converge, as $R \to \infty$, to the eigenvalue statistics near $1$ of a classical compact group, and that the limit depends on the family only through its symmetry type. We study the first correction to this limit for families of holomorphic cusp newforms of fixed weight $k$ and varying level $N$. Sharpening work of Miller on lower order terms in the one-level density, we evaluate the harmonically weighted one- and two-level densities with errors $O\left(\log^{-5}(R)\right)$ and $O\left(\log^{-2}(R)\right)$, and show that each of them already differs at order $\log^{-1}(R)$ from an explicit universal profile built out of $k$, the test functions, and $R$ alone. We compute that difference exactly. It is the product of a functional of the test functions with a single arithmetic invariant $\kappa_1(F)$ of the family, an explicit sum over the bounded prime factors of the level. Two families of newforms of the same weight and the same symmetry type, with conductors of the same size, therefore have densities whose first lower order terms differ by an explicit nonzero amount whenever their levels have different bounded prime factors.

==> abstract.tex <==

\begin{abstract}
The Katz-Sarnak density conjecture states that, as the analytic conductor $R \to \infty$, the distribution of the normalized low-lying zeros of a family of $L$-functions converges to the scaling limits of eigenvalues clustered near 1 of subgroups of $U(N)$. Evidence shows that this conjecture holds in many families, including the family of holomorphic cusp newforms. In 2009, Miller computed lower-order terms for the 1-level density of some $GL(2)$ families. We extend his work by identifying family-dependent lower-order correction terms in the weighted 1-level and 2-level densities of holomorphic cusp newforms up to $O\left(1/\log^4 R\right)$ error, sharpening Miller's $O\left(1/\log^3 R\right)$ error. We show that the rates at which the prime factors of the level tend to infinity lead to different lower-order terms, breaking the universality of the main behavior and illuminating the arithmetic of the family. 
\end{abstract}
